PipeFill: Using GPUs During Bubbles in Pipeline-parallel LLM Training

Training Deep Neural Networks (DNNs) with billions of parameters generally involves pipeline-parallel (PP) execution. Unfortunately, PP model training can use GPUs inefficiently, especially at large scale, due to idle GPU time caused by pipeline bubbles, which are often 15-30% and can exceed 60% of the training job's GPU allocation. To improve the GPU utilization of PP model training, this paper describes PipeFill, which fills pipeline bubbles with execution of other pending jobs. By leveraging bubble GPU time, PipeFill reduces the GPU utilization sacrifice associated with scaling-up of large-model training. To context-switch between fill jobs and the main training job with minimal overhead to the main job, and maximize fill job efficiency, PipeFill carefully fits fill job work to measured bubble durations and GPU memory availability, introduces explicit pipeline-bubble instructions, and orchestrates placement and execution of fill jobs in pipeline bubbles. Experiments show that PipeFill can increase overall utilization by up to 63% for GPUs used in large-scale LLM training, with <2% slowdown of the training job, and 5-15% even for low-scale LLM training. For large-scale LLM training on 8K GPUs, the 63% increase translates to up to 2.6K additional GPUs worth of work completed.

==> design.tex <==
\section{\sysname Design}
\label{sec:design}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/system_overview.pdf}
  
  \vspace{4pt}
  \scriptsize
  \textbf{Dev}: Device \quad
  \textbf{Exec}: Execution
  \vspace{-4pt}
  
  \caption{System overview}
  \label{fig:system_overview}
\end{figure}

\subsection{\sysname Architecture}
To address the main challenges in \ref{subsec:challenges}, \sysname introduces three major components built on top of existing hybrid-parallel systems: a fill-job Placer, a pipeline-stage Coordinator, and a pipeline-bubble instruction.
Figure~\ref{fig:system_overview} shows the system overview of \sysname.
Fill jobs are initially received by the Placer, which decides which pipeline-stage Coordinator's queue to place the job in.
%
Each pipeline-stage Coordinator resides on the machine which holds the rank-1 pipeline-stage replica.
A Coordinator manages all device workers in a single pipeline-stage.
A Coordinator orders the fill jobs in its queue according to a policy, and for every job it uses profiling data to construct an execution plan.
%
Each execution plan describes which device the job will execute on, when it will execute, and how it will be executed without violating the bubbles' constraints.
%
To enable the Coordinators to create execution plans for fill-jobs whose entire models do not fit in the pipeline-bubble free-memory, and to exploit the differences in free-memory between different bubble types, \sysname partitions fill-job models using a Partitioning Algorithm that considers bubble lengths and free-memory in order to minimize fill-job execution time.
%
The pipeline engine, which runs on every device worker, receives executable jobs from the Coordinator to run during pipeline bubbles.
The pipeline engine uses the pipeline bubble instruction to know when a pipeline bubble is beginning so it can execute the fill jobs.
The pipeline engine returns to the Coordinator whenever it has completed some work, so the Coordinator can know the progress of all the fill jobs and allocate more work to continue filling the pipeline bubbles.
%
All together the system introduces:
\begin{itemize}[leftmargin=3mm,noitemsep,nolistsep]
  \setlength{\itemsep}{-0pt}
    \item Pipeline bubble instructions to know when to context-switch between fill jobs and the main job.
    \item A job Placer and Coordinator to decide exactly which job to run on which devices' bubbles.
    \item A Partitioning algorithm to enable optimal execution of jobs on pipeline bubbles with duration and memory constraints.
\end{itemize}

% To address the main challenges in \ref{subsec:challenges}, \sysname introduces three major components built on top of existing hybrid-parallel systems: a fill-job Scheduler, a pipeline-stage Coordinator, and a pipeline-bubble instruction, shown in Figure~\ref{fig:system_overview}. The pipeline-engine uses the bubble instruction to 1) measure the bubble durations and free memory and 2) know when a pipeline bubble is beginning so it can execute the fill jobs. The pipeline engine receives executable jobs from the Coordinator, which manages all device workers (each with an instance of the pipeline engine) in a single pipeline-stage. The Coordinator resides on the machine which holds the rank-1 pipeline-stage replica. The Coordinator creates an execution plan for all unfinished jobs that are submitted to it. \zhen{is the coordinator placed in on a standalone machine as a centralized controller or?} \daiyaan{its on the rank-1 replica}Together with the Scheduler, which receives the arriving fill-job requests and decides which Coordinator to submit them to, the Coordinators' execution plans describe which device the jobs will execute on, in what order they will execute, and how they will be executed without violating the bubbles' constraints. \zhen{so logically, the scheduler sec4.4 receive the job from user, then submit then to different coordinators, then we probably want to mention the scheduler first.} To enable the Coordinators to execute fill-jobs whose entire models do not fit in the pipeline-bubble free-memory and to exploit the differences in free-memory between different bubble types, PipeFill partitions fill-job models using a Partitioning Algorithm that considers bubble lengths and free-memory in order to minimize fill-job execution time. \daiyaan{add overview figure, explain design decisions/key ideas corresponding to exact challenges in the motivation} \zhen{adding the section reference for each compoenent.}

% \sysname introduces a new pipeline instruction and two major components built on top of existing hybrid-parallel systems: a fill-job Scheduler and a pipeline-stage Coordinator. \sysname creates a new bubble instruction for existing pipeline engines to indicate when to execute fill jobs. The bubble instruction receives executable jobs from the Coordinator, which manages all device workers (each with an instance of the pipeline engine) in a single pipeline-stage. The Coordinator creates an execution plan for all unfinished jobs that are submitted to it; the execution plan describes when and how each job will execute and on which device worker. The Scheduler receives the arriving fill-job requests, and decides which Coordinator to submit
% the job to. When a new job is submitted to a Coordinator, it modifies the existing plan to include the new job. To enable the Coordinators to execute fill-jobs whose entire models do not fit in the pipeline-bubble free-memory and to exploit the differences in free-memory between forward-bubbles and backward-bubbles, PipeFill partitions fill-job models using a Partitioning Algorithm that considers bubble lengths and free-memory in order to minimize fill-job execution time. \daiyaan{add overview figure, explain design decisions/key ideas corresponding to exact challenges in the motivation}

\subsection{Pipeline Engine Instrumentation}
In order to not impact the main job, we must keep the context switching and execution of fill jobs completely within the duration of the pipeline bubbles. We must also know exactly how much GPU memory the fill job can use during its execution so that the main job does not experience an OOM error. In order to achieve this, \sysname augments existing pipeline engines with a new pipeline bubble instruction. Existing pipeline engines execute a sequence of pipeline instructions. These instructions include sending/receiving activations and gradients, executing forward/backward computations on specific microbatches, and synchronizing parameters. Taken together as a periodically repeating sequence, these instructions constitute a pipeline schedule, which can have multiple pipeline bubbles which appear as instructions that wait on some event (e.g. activation data to arrive from the previous stage). \sysname's bubble instruction is inserted into the schedule to indicate where large bubbles are expected to occur. \par
\noindent \textbf{Bubble characterization.} Before doing any bubble filling, the pipeline engine must determine the time duration of each pipeline bubble in the pipeline schedule and how much memory is available for the fill jobs to use. To this end, at the beginning of the main training job the pipeline engine does profiling. For each bubble instruction, the pipeline engine will wait x amount of time (e.g. 100 ms) before proceeding to execute the next instruction. It will then observe the main job's throughput, if it is unaffected then on the next minibatch iteration it will wait 2x amount of time. This will continue until the pipeline engine observes a drop in  the main job's throughput, at which point it will know the duration of the pipeline bubble.
%\zhen{So this is an iterative process for profiling the time span of a bubble? if so, can we summarize it into an algorithm.}
%\mason{Is this G-pipe? Does our system only support G-pipe?}
%
To profile the amount of memory available for the engine to use for the fill job during a pipeline bubble, the engine relies on PyTorch's torch.cuda.memory\_allocated() function to know how much memory is held by the main training job during the bubble; the remaining device memory is considered free, but to ensure there are no out-of-memory errors \sysname may opt only to allocate some fraction of the free memory. \par
Once the pipeline bubble durations and free memory are known, the pipeline engine passes this information to its corresponding Coordinator. The pipeline engine also asks its Coordinator exactly what work to perform (i.e. which layers of which model to execute on which inputs) during its pipeline bubbles. To reduce the frequency with which it must communicate with the Coordinator, it asks for enough work to fill several pipeline bubbles, and when it runs out of work it asks the Coordinator for more work once again. The number of future pipeline bubbles the engine seeks to fill at a time is fixed and the same for all device workers. \par
\noindent \textbf{Fill job execution.} The executables dispatched to the engine by the Coordinators take the form of a torch.nn.Sequential instance with additional information to support parallelism and memory-reduction techniques. For our partitioned-execution technique, the executable contains the partition boundaries (which are just layer indices in the Sequential model) and the batch sizes to use for each partition during each pipeline bubble.
The engine iterates through the partitions; each partition executes during the bubbles, using the specific batch sizes and for the number of samples determined by the Coordinator, until it has finished executing all the samples sent by the Coordinator.
To preserve memory, all the outputs of executing a partition are offloaded to CPU memory and loaded back to GPU memory when the next partition is executed. When the last partition completes execution on all the samples, the engine asks the Coordinator for more work. If the Coordinator determines that the next executable that will be sent to the engine is the same as the one it just completed running, it will only send the next subset of samples and tell the engine to reuse the current executable; otherwise it will send a new executable with the new subset of samples. 

\subsection{Pipeline-Stage Coordinator}
The Coordinator manages all the GPUs in a single pipeline stage, and creates an execution plan for all the remaining jobs that have been assigned to it. The Coordinator's role is two-fold: it partitions the fill job models so they can fit in the free memory available to the fill jobs during the pipeline bubbles, and it determines which devices to execute the fill jobs on and in what order to execute them.
%\zhen{The first part states that the coordinator manages devices belonging to a pipeline stage, if so all these devices have the same bubble characteristic, then the last statement of ``it determines which devices ...'' does not make much sense. } \daiyaan{this means for DP or PS, described in "job ordering" subsection}
\par
\noindent \textbf{Executable construction.} The Coordinator receives the pipeline bubble configuration (bubble durations and free memory) from the engines. Since all the device workers assigned to a Coordinator belong to the same pipeline-stage, they all share the same bubble configuration. Therefore, the Coordinator must construct a single executable for a job that is submitted to it, and it can distribute the executable to any device worker that is assigned any samples of that job. To construct the executables, the Coordinator relies on profiles of the fill job model's layer execution times and memory consumption.
The executable describes how to partition a model and how to execute those partitions on a set of samples during the pipeline bubbles. For example, it may partition the model layers and execute each partition on the entire set of samples while dynamically adjusting the batch size according to the amount of memory available to a specific bubble to maximize throughput.
%\zhen{do you mean that bubbles are different in forward and backward computation?}\daiyaan{yes, they can have different free-memory and duration}
Other forms of partitioning (e.g. model-parallelism) and dynamic memory-reduction techniques (e.g. CPU-offloading, activation checkpointing) can also be considered by the Coordinator when constructing the executable. Finally, the executable also respects the pipeline bubble durations by specifying exactly how many samples to process in any given bubble. \par
\noindent \textbf{Partitioning algorithm.} To enable execution of models that do not fit in the GPU free memory and exploit the difference in GPU free memory between different bubbles in a pipeline schedule, we propose a new partitioning algorithm. The free variables which our algorithm aims to optimize are the layer-boundaries of the partitions and the batch sizes used to execute each partition during each bubble. The algorithm sets these variables to values that optimize the throughput of the fill job. To do this, we notice that this problem has an optimal-substructure property. The structure is the following: \\
$$T(k) = \min\limits_{i<k} \{ T(i) + \min\limits_{e\in \mathbb{N}^{2 \times P}} \text{TPS}(i+1, k, e) \}$$
where $T(i)$ is the lowest possible time-per-sample (inverse of throughput) for executing all layers up to layer i, $\text{TPS}(i+1, k, e)$ is the time-per-sample of executing layers i+1 to k as one partition using execution plan $e$. A plan $e$ describes what batch size to use when executing the partition for each pipeline bubble and how many batches to execute during each bubble. If a plan $e$ violates the memory constraints or duration of a bubble, $TPS$ returns infinity so that plan is not considered.
%\mason{Should we also formulate the memory constraints?} \daiyaan{this is basically provided in the profiles}
\par
This optimization problem can be solved using dynamic-programming. The complexity of the DP is $\mathcal{O}(L^2\times(BS)^P)$ where $L$ is the number of layers, $B$ is the number of batch sizes considered, $S$ is the number of samples considered, and $P$ is the number of pipeline bubbles. On first glance this complexity seems too high, but most of the terms an be bounded using heuristics. $L^2$ is bounded by the maximum number of layers any fill-job model can have. $B$ and $S$ are bounded by bubble constraints: $B$ is bounded by both the maximum free memory in any bubble and the maximum bubble duration, and $S$ is bounded by the maximum bubble duration. Additionally, we only consider powers of 2 for $B$
%\zhen{why is that?}\daiyaan{just because of convention}
, and $S$ can only be a multiple of $B$. $P$ is bounded by the maximum number of bubbles per minibatch iteration of the main job that the system tries to fill and is determined by the pipeline schedule; for GPipe $P=2$, and $P=2$ is typically enough to recover most of the pipeline bubble time. \par
\noindent \textbf{Job ordering.} The Coordinator orders the jobs according to the policy, such as First-In-First-Out (FIFO) and  Shortest-Job-First (SJF), before dispatching them to the device workers. This policy can be co-defined with the Placer's scoring function. Since the Coordinator manages multiple devices, it is desirable to also enable data parallel execution of jobs across the devices as well as concurrently running different jobs across different workers. Both of these can be naturally achieved by partitioning the samples of a job and ordering the sample partitions in the queue from which they are dispatched. \par Consider a Coordinator managing two devices with two jobs currently in submission. To execute the first job to completion using data parallelism followed by the second job, the ordering could be the following:
$$[(J_1, (1, 10)), (J_1, (11, 20)), ..., (J_2, (0, 10)), (J_2, (11, 20)), ...]$$ 
where $(J_i, (N_1, N_2))$ is the job partition of processing samples $N_1$ to $N_2$ of job $i$.
As the Coordinator dispatches work from the head of the queue, it will dispatch data-parallel partitions of $J_1$ to all of its workers. Once all of the $J_1$ partitions have been dispatched, it will do the same to $J_2$. Alternatively, to concurrently run both jobs, the ordering could be the following:
$$[(J_1, (1, 10)), (J_2, (0, 10)), (J_1, (11, 20)), (J_2, (11, 20)), ...]$$
The Coordinator will alternate between dispatching data-parallel partitions of $J_1$ and data-parallel partitions of $J_2$, concurrently running both jobs on its workers. \par
\noindent \textbf{Job arrival and dispatch} The fill job partitions/executables and their order in the queue constitutes the Coordinator's execution plan. Once the job executables are constructed and ordered, the Coordinator dispatches them to the device workers. Recall that each engine periodically requests work from its Coordinator to fill its bubbles. When the Coordinator receives such a request, it will send a job executable and a subset of that job's total remaining samples to be run on that engine's device. The Coordinator may also dispatch these (executable, subset) pairs in parallel to multiple engines when the executable includes any parallelism. When a new job is submitted to the Coordinator, it constructs an executable for the new job and determines how to partition the dataset and how to place the new job's (executable, subset) pairs in the existing ordering; the queue with the new job's partitions inserted is the Coordinator's new execution plan.

\subsection{Placer}
The Placer has a user-defined scoring function which takes every Coordinator's execution plan (order of fill job partitions in the queue) as input and outputs a score. As stated, the execution plan describes how every fill job will run. This information can be used to calculate each job's queueing time, completion time, and efficiency. The scoring function uses these job values to optimize a cluster-wide metric; any cluster-wise metric that is a function of the job values can be used, such as average job completion time (JCT), 99th percentile JCT, makespan, fairness, and efficiency.
\par
When a new job arrives, the Placer queries each pipeline-stage Coordinator for its current workload and what its execution plan would be if the new job were added to its workload. Using the scoring function, the Placer routes the new job to whichever Coordinator is optimal. If the Placer did not directly query each Coordinator, and instead used some heuristic to determine which Coordinator to submit to in order to optimize the score, it would miss out on the critical information of how different Coordinators' bubbles differ and how that affects the performance of each job. Each Coordinator manages an entire pipeline-stage, so while all the devices managed by a single Coordinator experience identical pipeline bubbles (which also occur at the same time), devices managed by different Coordinators can vary substantially in their pipeline bubbles. This information is critical to know since some jobs can be completed much quicker on some Coordinators, while others complete in nearly the same time no matter which Coordinator they are submitted to. \par
As an example, consider a Placer whose scoring function is the following: $$f(p_1, ..., p_c) = \frac{\sum_{i=1}^{c}\sum_{k \in p_i} JCT(J_k)}{\sum_{i=1}^{c} \vert p_i \vert}$$
where $p_i$ is the execution plan of Coordinator $i$. The score achieved is equal to the average JCT, which the Placer aims to minimize. When a new job arrives, the Placer will recalculate the score for each Coordinator with the new job added to its plan, and choose the Coordinator whose score (average JCT) increases the least: 
$$\arg \min_i \sum_{k \in insert(p_i, J_{new})}JCT(J_k) - \sum_{k \in p_i}JCT(J_k)$$
The Placer is the single point of interface between entities who wish to submit jobs to execute on the pipeline bubbles and the instance of \sysname managing the pipeline bubbles of a training job. An overarching cluster scheduler could interface with the Placer to treat the main training job's bubbles as another resource (in addition to the other resources under its management) to schedule jobs on. 


==> eval.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{0.4\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/main/main_flops.pdf}
    %\vspace{.3pt}
    \caption{FLOPS breakdown}
    \label{fig:main_flops}
    \vspace{-10pt}
  \end{subfigure}
  \hspace{2mm}
  %
  \begin{subfigure}{0.4\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/main/main_time.pdf}
    %\vspace{.3pt}
    \caption{GPU-time breakdown}
    \label{fig:main_time}
    \vspace{-10pt}
  \end{subfigure}
  %
  \caption{
  FLOPS and GPU-time breakdown with and without \sysname at different main job (i.e., LLM) scales.
  The red bars represent traditional execution, where pipeline bubbles are wasted GPU time.
  The blue bars represent \sysname{}-managed execution, with the cross-hatch portion indicating the fill job portion.
  Note that the LLM achieves the same FLOPS (and GPU time) in both cases.
  }
%  \vspace{-25pt}
\end{figure*}

\section{Evaluation}
\label{sec:eval}

Our experimental results confirm that \sysname{} can successfully utilize the GPU time traditionally wasted by pipeline bubbles in large-scale DNN training.
We organize this section into four parts:
\begin{enumerate}[leftmargin=3mm,noitemsep,nolistsep]
  \setlength{\itemsep}{-0pt}
  \item
    Main results: showing GPU utilization with and without \sysname as a large LLM is scaled from using 8K to 32K GPUs (Sec. \ref{sec:eval:main}); 
  \item
    Benefit attribution: measuring the incremental impact of \sysname's components: coordinator policy, partitioning algorithm and placer (Sec. \ref{sec:eval:attr}); 
  \item
    Ablation studies: evaluating the impact of free memory quantity in bubbles and fill job model types (Sec. \ref{sec:eval:ablation}); 
  \item
    Simulator fidelity: validating that the simulator reflects reality accurately enough to make its results meaningful (Sec. \ref{sec:eval:sim}).
\end{enumerate}

\subsection{Main Results}
\label{sec:eval:main}

%\mason{Need to highlight our main claim is that our system improve the cluster GPU utilization without sacrificing the main job's performance.}
%\mason{Where did we get this result? Can we explicitly place it somewhere in the main result?
%"the training time of a 40B parameter LLM can be reduced by over 1 week by scaling from 8K to 32K."
%} \daiyaan{added statement in simulator section stating all our results are from the simulator}

We show that \sysname recovers most of the wasted GPU resources from scaling large model training with little overhead to the main job. Figure \ref{fig:main_flops} breaks down the total GPU FLOPS used by the main job and by the fill jobs on the main job's bubbles in a cluster of 32K GPUs as we scale the main job from using 8K to 32K GPUs. As we scale the main job without filling, the main job takes exclusive ownership of an increasing fraction of the cluster GPUs. The majority of these FLOPS are wasted since as the main job scales up its pipeline bubble ratio increases. Most of the wasted FLOPS are recovered by filling the main job's bubbles with fill jobs, at a small ($<5\%$) cost to the main job. \par
Figure \ref{fig:main_time} shows a breakdown of GPU-time received in the same setup. The GPU-time received by the main job increases proportionally more than the FLOPS it uses; this is because the efficiency of the main job decreases as it is scaled up (independent of pipeline bubbles). However, the total amount of GPU-time wasted still increases due to the pipeline bubbles; most of this wasted GPU-time is recovered by \sysname.  While the fill jobs run at a reduced efficiency in the bubbles than on exclusive GPUs (due to memory and duration constraints of bubbles), their aggregate throughput is only reduced by up to 30\%. However, when comparing filling with no-filling at the highest main job scale, we see a 1.9x increase in FLOPS utilization while increasing the main job throughput by 40\% compared to the lowest scale. 

% Figure \ref{fig:main} shows the GPU utilization (in HFU) of a XXB parameter LLM pretraining job as we increase the number of GPUs that the job is run on (by increasing the amount of data parallelism). As expected, the HFU steadily decreases due to the increase in pipeline bubbles. By filling the pipeline bubbles, we recover enough GPU utilization to keep the HFU close to constant as we scale up the main job. \daiyaan{we can replace this figure with a breakdown of flops consumed and GPU hours consumed by main job vs fill jobs}



%\begin{figure}[t]
%\centering
%\includegraphics[width=7cm,keepaspectratio]{figs/main/main_flops.pdf}
%\caption{
%Cluster FLOPS breakdown with and without \sysname at different scales.
%}
%\label{fig:main_flops}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=7cm,keepaspectratio]{figs/main/main_time.pdf}
%\caption{
%Cluster GPU-time breakdown with and without \sysname at different scales.
%}
%\label{fig:main_time}
%\end{figure}

% To measure the efficiency with which the fill jobs can use the bubbles, in Figure \ref{fig:fill} we compare the fill jobs' throughput on an exclusive cluster of 8K GPUs to the fill jobs' throughput executing only in the bubbles of an LLM training job on 16K GPUs. Executing on the bubbles, the fill jobs' receive 1.36x the GPU resources (in GPU execution time) and achieve 1.23x the throughput compared to the exclusive cluster; therefore the fill jobs run at over 90\% of the efficiency they receive on the exclusive cluster by running in the pipeline bubbles. 

% \begin{figure}[h]
% % \caption{\textcolor{red}{do dp=32 to dp=64}}
% \caption{fill job throughput as main job allocation is increased}
% \centering
% \label{fig:fill}
% \includegraphics[width=8cm,keepaspectratio]{figs/main/fill_scale.pdf}
% \end{figure}

%\subsection{Simulator fidelity}
%To validate the accuracy of the simulator, we measure the execution time of the main job with and without \sysname. We run with a trace of only swin-L jobs of the same size, since we are measuring the system execution performance (which does not depend on the trace); note that swin models are much less efficient than other models in our trace (e.g. bert, wide-resnet). We seed the simulator with the profiles of executing without \sysname with 32K GPUs. In Figure \ref{fig:sim_flops} we plot real and predicted FLOPS breakdown of the main/fill jobs with and without \sysname at different scales. Despite only being seeded with profiles of the main job without \sysname at 32K GPUs, the simulator predicts every component of the FLOPS breakdowns with $<11\%$ error. In Figure \ref{fig:sim_tput}, we plot the real and predicted main job throughput at different scales with and without \sysname; the simulator again predicts the throughput with $<8\%$ across all scales. This close match allows us to use to simulator to evaluate \sysname{}'s behavior and benefits across scales and configurations that would not be feasible (for research explorations) otherwise.
%
%\begin{figure}[h]
%\caption{}
%\centering
%\includegraphics[width=8cm,keepaspectratio]{figs/sim_phy/sim_fid.pdf}
%\label{fig:sim_flops}
%\end{figure}
%
%\begin{figure}[h]
%\caption{}
%\centering
%\includegraphics[width=8cm,keepaspectratio]{figs/sim_phy/sim_fid_main_tput.pdf}
%\label{fig:sim_tput}
%\end{figure}

\subsection{Attribution of Benefits}
\label{sec:eval:attr}

We now analyze the impact of the different components of \sysname's design. We show how the Coordinator's queuing policy can affect different fill job metrics that may be of interest, how the partitioning algorithm improves the efficiency with which the fill jobs execute in the pipeline bubbles, and how the Placer's action of ``matching'' jobs to the correct pipeline stage (due to bubble differences) also improves efficiency. \par
For the partitioning algorithm and Placer evaluation, we reduce the forward-bubble free-memory to 0.5GB, which can occur if the main job reduces activation-checkpointing\cite{korthikanti2023reducing} to create a large imbalance between the forward and backward bubbles. This showcases the benefit of the partitioning algorithm and the Placer, since they are designed precisely to handle such imbalances. \par
\noindent \textbf{Coordinator policy.} First, we show how the Coordinator policy can be adjusted to optimize certain metrics. We use two different policies for the Coordinator: FIFO and SJF. In Figure \ref{fig:coord_policy}, we plot the average JCT and 99th percentile JCT of both policies as the arrival rate is scaled. SJF maintains a low average JCT, but FIFO has a substantially lower 99th percentile JCT at higher arrival rates. More specific policies (e.g. PS, max-min-fairness) can be implemented at the Coordinator to optimize other metrics. \par
\noindent \textbf{Partitioning algorithm.} We now show that our partitioning algorithm improves the efficiency of the fill jobs' execution. Figure \ref{fig:eff} shows the CDF of HFU achieved by fill jobs with and without our partitioning algorithm. The baseline uses a fixed batch size for all partitions to use on all bubbles and creates the largest possible partitions that can execute that batch size without running out of memory (the batch size is optimized). We can see that our partitioning algorithm improves the HFU of all jobs, and in particular the jobs with the lowest HFU see a significant improvement. In Figure \ref{fig:eff_box}, we show the efficiency of the fill jobs split by their model types; the jobs that our partitioning algorithm improves the efficiency of the most are the jobs running Swin and XLM models. \par
\noindent \textbf{Placer.} We now show that our Placer design (querying the Coordinators for the execution plans before submitting a new job) vastly outperforms a non-Coordinator-aware Placer. In Figure \ref{fig:sched} we compare the Placer submitting jobs with three different strategies: round-robin over the Coordinators, submit to the shortest-queue Coordinator, and \sysname (which queries the Coordinator's for their execution plans). We plot the average GPU-hours consumed to complete XLM jobs and non-XLM jobs for each Placer. We see that the benefit of the Placer comes mainly from placing the large XLM jobs on the optimal Coordinators. 

\begin{figure}[t]
\centering
\includegraphics[width=7cm,keepaspectratio]{figs/attribution/coord_design.pdf}
\caption{JCT comparison between two different SJF and FIFO coordinator policies.}
\label{fig:coord_policy}
\end{figure}

\begin{figure}[t]
% \caption{\textcolor{red}{add exclusive cluster flop dist to this}}
\centering
\includegraphics[width=8cm,keepaspectratio]{figs/attribution/cdf.pdf}
\caption{CDF of fill job HFUs with and without partitioning algorithm.}
\label{fig:eff}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=7cm,keepaspectratio]{figs/attribution/eff_box.pdf}
\caption{TFLOPS utilization with and without partitioning algorithm.}
\label{fig:eff_box}
\end{figure}

\begin{figure}[t]
% \caption{\textcolor{red}{use bubble partition for this}}
\centering
\includegraphics[width=7cm,keepaspectratio]{figs/attribution/sched_eff.pdf}

\vspace{4pt}
\scriptsize
  \textbf{RR}: Round-Robin \quad
  \textbf{SQ}: Shortest-Queue \quad
  \textbf{PF}: \sysname

\caption{Average GPU-hours consumed to complete fill jobs using different Placer strategies.}
\label{fig:sched}
\end{figure}

\begin{figure*}[t!]
  \centering
  \begin{subfigure}{0.4\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid.pdf}
    %\vspace{.3pt}
    \caption{FLOPS breakdown}
    \label{fig:sim_flops}
    \vspace{-10pt}
  \end{subfigure}
  \hspace{2mm}
  %
  \begin{subfigure}{0.40\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid_main_tput.pdf}
    %\vspace{.3pt}
    \caption{Main job throughput}
    \label{fig:sim_tput}
    \vspace{-10pt}
  \end{subfigure}
  %
  \caption{
  Real v.s. simulated FLOPS breakdown and main job throughput with and without \sysname at different scales.
  }
%  \vspace{-25pt}
\end{figure*}

\subsection{Ablations}
\label{sec:eval:ablation}

We do several ablations on different system parameters. \par
\noindent \textbf{Free memory quantity in bubbles.} Free memory capacity can be affected by several things such as how aggressively the main job checkpoints activations to reduce memory overhead, the main job's model size and optimizer, and how much the main job state is partitioned vs replicated vs offloaded.  \par
In Figure \ref{fig:free_mem} we fix one bubble type's free-memory and vary the other bubble type's free memory. On one line, we fix the forward-bubble free-memory at 0.5GB and increase the backward-bubble free-memory from 1.5GB to 3 GB; on the other line we hold the backward-bubble free-memory at 1.5GB and increase the forward-bubble free-memory from 0.5GB to 1.5GB. The results show that increasing the minimum bubble free-memory increases efficiency (by decreasing average GPU-hours to complete each fill job) substantially, while increasing the maximum bubble free-memory does not affect efficiency. This may be because with less memory the fill jobs must execute with smaller partitions which incurs a larger activation offloading overhead and results in partitions that are too small to saturate the GPU compute. \par
\noindent \textbf{Fill job model-types.} Among the model types in our traces, the largest models incur much larger memory overheads (both in parameters and activations) than other models, and this in-turn reduces those models' execution efficiency on pipeline bubbles. To evaluate the impact of these large-model fill jobs, we replace a fraction of the large-model jobs with medium-model jobs (without changing the job-size distribution in GPU-hours or the arrival rate of jobs). As we increase this fraction, the average JCT is reduced substantially; replacing 20\% of the large-model jobs reduces the average JCT from 3.97 hours to 0.76 hours. This analysis informs how an overarching cluster scheduler could decide which jobs to submit to the \sysname Placer to execute on pipeline bubbles. 

\begin{figure}[t]
% \caption{\textcolor{red}{use bubble partition for this}}
\centering
\includegraphics[width=6.6cm,keepaspectratio]{figs/ablations/free_mem.pdf}
\caption{Ablation study: free memory quantity in bubbles.}
\label{fig:free_mem}
\end{figure}

% \begin{figure}[h]
% \caption{\textcolor{red}{use bubble partition for this}}
% \centering
% \includegraphics[width=7cm,keepaspectratio]{figs/ablations/fill_model_dist.pdf}
% \caption{Ablation study: fill job model-types.}
% \label{fig:fill_dist}
% \end{figure}

% \begin{figure*}[b!]
%   \centering
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid.pdf}
%     %\vspace{.3pt}
%     \caption{FLOPS breakdown}
%     \label{fig:sim_flops}
%     \vspace{-10pt}
%   \end{subfigure}
%   \hspace{2mm}
%   %
%   \begin{subfigure}{0.40\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid_main_tput.pdf}
%     %\vspace{.3pt}
%     \caption{Main job throughput}
%     \label{fig:sim_tput}
%     \vspace{-10pt}
%   \end{subfigure}
%   %
%   \caption{
%   Real v.s. simulated FLOPS breakdown and main job throughput with and without \sysname at different scales.
%   }
% %  \vspace{-25pt}
% \end{figure*}

\subsection{Simulator Fidelity}
\label{sec:eval:sim}

To validate the accuracy of the simulator, we measure the execution time of the main job with and without \sysname. We run with a trace of only Swin-L jobs of the same size, since we are measuring the system execution performance (which does not depend on the trace); note that Swin models are much less efficient than other models in our trace (e.g. bert, Wide-ResNet). We seed the simulator with the profiles of executing without \sysname with 32K GPUs. In Figure \ref{fig:sim_flops} we plot real and predicted FLOPS breakdown of the main/fill jobs with and without \sysname at different scales. Despite only being seeded with profiles of the main job without \sysname at 32K GPUs, the simulator predicts every component of the FLOPS breakdowns with $<11\%$ error. In Figure \ref{fig:sim_tput}, we plot the real and predicted main job throughput at different scales with and without \sysname; the simulator again predicts the throughput with $<8\%$ across all scales. The error on other scales and on simulating with \sysname can be further reduced by seeding the simulator with profiles collected in those environments, which is what we do for all of our other experiments. This close match allows us to use the simulator to evaluate \sysname{}'s behavior and benefits across scales and configurations that would not be feasible (for research explorations) otherwise.

% \begin{figure*}[b!]
%   \centering
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid.pdf}
%     %\vspace{.3pt}
%     \caption{FLOPS breakdown}
%     \label{fig:sim_flops}
%     \vspace{-10pt}
%   \end{subfigure}
%   \hspace{2mm}
%   %
%   \begin{subfigure}{0.40\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/sim_phy/sim_fid_main_tput.pdf}
%     %\vspace{.3pt}
%     \caption{Main job throughput}
%     \label{fig:sim_tput}
%     \vspace{-10pt}
%   \end{subfigure}
%   %
%   \caption{
%   Real v.s. simulated FLOPS breakdown and main job throughput with and without \sysname at different scales.
%   }
% %  \vspace{-25pt}
% \end{figure*}

%\begin{figure}[t]
%\centering
%\includegraphics[width=7cm,keepaspectratio]{figs/sim_phy/sim_fid.pdf}
%\caption{
%Real v.s. simulated FLOPS breakdown with and without \sysname at different scales.
%}
%\label{fig:sim_flops}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=7cm,keepaspectratio]{figs/sim_phy/sim_fid_main_tput.pdf}
%\caption{
%Real v.s. simulated main job throughput with and without P\sysname at different scales.
%}
%\label{fig:sim_tput}
%\end{figure}

==> other-guidance.tex <==
%-------------------------------------------------------------------------------
\section{Footnotes, Verbatim, and Citations}
%-------------------------------------------------------------------------------

Footnotes should be places after punctuation characters, without any
spaces between said characters and footnotes, like so.%
\footnote{Remember that USENIX format stopped using endnotes and is
  now using regular footnotes.} And some embedded literal code may
look as follows.

\begin{verbatim}
int main(int argc, char *argv[]) 
{
    return 0;
}
\end{verbatim}

Now we're going to cite somebody. Watch for the cite tag. Here it
comes. Arpachi-Dusseau and Arpachi-Dusseau co-authored an excellent OS
book, which is also really funny~\cite{arpachiDusseau18:osbook}, and
Waldspurger got into the SIGOPS hall-of-fame due to his seminal paper
about resource management in the ESX hypervisor~\cite{waldspurger02}.

The tilde character (\~{}) in the tex source means a non-breaking
space. This way, your reference will always be attached to the word
that preceded it, instead of going to the next line.

And the 'cite' package sorts your citations by their numerical order
of the corresponding references at the end of the paper, ridding you
from the need to notice that, e.g, ``Waldspurger'' appears after
``Arpachi-Dusseau'' when sorting references
alphabetically~\cite{waldspurger02,arpachiDusseau18:osbook}. 

It'd be nice and thoughtful of you to include a suitable link in each
and every bibtex entry that you use in your submission, to allow
reviewers (and other readers) to easily get to the cited work, as is
done in all entries found in the References section of this document.

Now we're going take a look at Section~\ref{sec:figs}, but not before
observing that refs to sections and citations and such are colored and
clickable in the PDF because of the packages we've included.

%-------------------------------------------------------------------------------
\section{Floating Figures and Lists}
\label{sec:figs}
%-------------------------------------------------------------------------------


%---------------------------
\begin{figure}
\begin{center}
\begin{tikzpicture}
  \draw[thin,gray!40] (-2,-2) grid (2,2);
  \draw[<->] (-2,0)--(2,0) node[right]{$x$};
  \draw[<->] (0,-2)--(0,2) node[above]{$y$};
  \draw[line width=2pt,blue,-stealth](0,0)--(1,1)
        node[anchor=south west]{$\boldsymbol{u}$};
  \draw[line width=2pt,red,-stealth](0,0)--(-1,-1)
        node[anchor=north east]{$\boldsymbol{-u}$};
\end{tikzpicture}
\end{center}
\caption{\label{fig:vectors} Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. }
\end{figure}
%% %---------------------------


Here's a typical reference to a floating figure:
Figure~\ref{fig:vectors}. Floats should usually be placed where latex
wants then. Figure\ref{fig:vectors} is centered, and has a caption
that instructs you to make sure that the size of the text within the
figures that you use is as big as (or bigger than) the size of the
text in the caption of the figures. Please do. Really.

In our case, we've explicitly drawn the figure inlined in latex, to
allow this tex file to cleanly compile. But usually, your figures will
reside in some file.pdf, and you'd include them in your document
with, say, \textbackslash{}includegraphics.

Lists are sometimes quite handy. If you want to itemize things, feel
free:

\begin{description}
  
\item[fread] a function that reads from a \texttt{stream} into the
  array \texttt{ptr} at most \texttt{nobj} objects of size
  \texttt{size}, returning returns the number of objects read.

\item[Fred] a person's name, e.g., there once was a dude named Fred
  who separated usenix.sty from this file to allow for easy
  inclusion.
\end{description}

\noindent
The noindent at the start of this paragraph in its tex version makes
it clear that it's a continuation of the preceding paragraph, as
opposed to a new paragraph in its own right.


\subsection{LaTeX-ing Your TeX File}
%-----------------------------------

People often use \texttt{pdflatex} these days for creating pdf-s from
tex files via the shell. And \texttt{bibtex}, of course. Works for us.

%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

The USENIX latex style is old and very tired, which is why
there's no \textbackslash{}acks command for you to use when
acknowledging. Sorry.

%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.

==> outline.tex <==
\section{Outline}
contributions: 
\begin{itemize}
    \item we recover GPU utilization by filling pipeline bubbles with our proposed fill-job execution techniques; we support batch inference fill jobs for model sizes up to 2B parameters without affecting the main jobs ($<15\%$ impact on throughput)
    \begin{itemize}
        \item for batch-inference fill jobs, we exploit the difference in free-memory between forward and backward bubbles by dynamically adjusting batch size and activation buffer size depending on the bubble type \zhen{Can we formulate this process as a scheduling algorithm with clear definition of inputs and outputs?}
        \item we partition the model layers to maximize throughput of our execution strategy depending on the relative size of forward/backward bubbles of the device a job is scheduled on \zhen{Is this part of the input to the algorithm mentioned in the last item?}
        \item we schedule jobs to devices according to their improved utility (due to larger backward bubbles i.e. more bubble time with larger free memory) 
        \item (tentative) we increase the memory available to the fill-jobs by offloading some memory of the main jobs; we prioritize offloading activations which can be swapped back by using parallel bandwidth of tensor-parallel GPUs (which share high bandwidth interconnect); for larger bubbles to further increase the free memory we offload weights and swap them back using parallel bandwidth of data-parallel GPUs; we coordinate the memory swapping with the execution of fill jobs to not affect the main jobs \zhen{If we formulate the free memory available on a device and the corresponding idle time (i.e., the bubble), can we expect the scheduling is general to this additional features? }
        \item (tentative) for training fill jobs, we exploit free-memory differences by dynamically adjusting the amount of activation checkpointing \zhen{The scheduling algorithm can general to this case, if we make the free memory and idle time as variables to the scheduling, and we can make the scheduling execution running multi-round }
    \end{itemize}
\end{itemize}
main results:
\begin{itemize}
    \item figure 1 (best result): show recovered HFU from filling with small model batch inference, breakdown of "time" filled vs "flops" filled (i.e. fill job HFU vs bubble time filled) \zhen{Can we make it more clear like what would be the x-axis and y-axis, are we going to show the HFU over a time period? how many baselines are we going to compare with?} \daiyaan{x-axis is data-parallel degree of main job, y-axis is HFU; it will be a bar plot showing the reduced HFU plus the recovered HFU}
    \item figure 2 (best result): show average JCT / "efficiency" of fill jobs compared to a resource-equivalent (in GPU hours) cluster with no main job, with/without memory space-sharing overhead \zhen{In addition to this figure, we can add one to should the throughput of the main job is not largely affected. } \daiyaan{I'll think more about how to show this, because I think the impact on the main job is relatively constant unless we add offloading}
    \item figure 3 (best result): main job slowdown, sources of slowdown, discussion of what can be done
    \item figure 4: show that its not a tradeoff for the main job, show that its performance is actually increasing as a function of total resources it consumes
\end{itemize}
ablations:
\begin{itemize}
    \item figure 3: free-memory vs throughput of fill jobs by changing batch size only, act buffer size only, and both \zhen{is this the ablation study to understand different system characteristic? }
    \item figure 4: show impact of correct model partition on free-memory vs throughput, forward/backward relative bubble size 
    \item figure 5: simulator fidelity
    \item figure 6: ablation of free-memory utilization, scheduling impact on JCT when fill job models are larger (but same job size distribution in GPU hours) \zhen{does this mean to experiment with different sized main training job? if so can we also list out the tentative target models?} \daiyaan{no, this is changing the fill jobs only; we can add another figure for different sized LLM main jobs}
\end{itemize}

\textbf{TODOs}
\begin{itemize}
    \item collect main results
    \item initial ablations of partitioning and scheduling algos against strongest baselines
\end{itemize}


